A Dual-Perspective Metaphor Detection Framework Using Large Language Models

Metaphor detection, a critical task in natural language processing, involves identifying whether a particular word in a sentence is used metaphorically. Traditional approaches often rely on supervised learning models that implicitly encode semantic relationships based on metaphor theories. However, these methods often suffer from a lack of transparency in their decision-making processes, which undermines the reliability of their predictions. Recent research indicates that LLMs (large language models) exhibit significant potential in metaphor detection. Nevertheless, their reasoning capabilities are constrained by predefined knowledge graphs. To overcome these limitations, we propose DMD, a novel dual-perspective framework that harnesses both implicit and explicit applications of metaphor theories to guide LLMs in metaphor detection and adopts a self-judgment mechanism to validate the responses from the aforementioned forms of guidance. In comparison to previous methods, our framework offers more transparent reasoning processes and delivers more reliable predictions. Experimental results prove the effectiveness of DMD, demonstrating state-of-the-art performance across widely-used datasets.

==> imgs/theory.tex <==
\begin{figure}[t]
\centering

    \includegraphics[width=0.9\linewidth]{imgs/Previous.pdf}

%
\caption{Two examples of metaphor detection using MIP and SPV theories. The MIP theory identifies metaphors by detecting conflicts between the word's basic and contextual meanings, as showed in (a). While the SPV theory pinpoints metaphors through the inconsistency between context and the selectional preference, as showed in (b).}
\label{fig:theory}
\vspace{-10pt}
\end{figure}
